Stellar population synthesis models at low and high redshift

The basic assumptions behind Population Synthesis and Spectral Evolution models are reviewed. The numerical problems encountered by the standard population synthesis technique when applied to models with truncated star formation rates are described. The Isochrone Synthesis algorithm is introduced as a means to circumvent these problems. A summary of results from the application of this algorithm to model galaxy spectra by Bruzual and Charlot (1993, 2000) follows. I present a comparison of these population synthesis model predictions with observed spectra and color magnitude diagrams for stellar systems of various ages and metallicities. It is argued that models built using different ingredients differ in the resulting values of some basic quantities (e.g. $M/L_V$), without need to invoking violations of physical principles. The range of allowed colors in the observer frame is explored for several galaxy redshifts.

==> cupdefs.tex <==
\ifoldfss
\else
  \ifnfssone
    \newmathalphabet{\mathit}
      \addtoversion{normal}{\mathit}{cmr}{m}{it}
      \addtoversion{bold}{\mathit}{cmr}{bx}{it}
    \newmathalphabet{\mathcal}
      \addtoversion{normal}{\mathcal}{cmsy}{m}{n}
    \else
    \ifnfsstwo
    \fi
  \fi
\fi

%%%%% USER-DEFINED MACROS HERE %%%%%
% Keep your own macro definitions separate from the examples below.
%
% Some useful examples of macro definitions follow.
%%%%%

\def\LaTeX{\lecurrentfam=\the\fam \leavevmode L\raise.42ex
\hbox{$\fam\lecurrentfam\scriptstyle\kern-.3em A$}\kern-.15em\TeX}
\def\plotone#1{\centering \leavevmode
\epsfxsize=\textwidth \epsfbox{#1}}
\def\plottwo#1#2{\centering \leavevmode
\epsfxsize=.45\textwidth \epsfbox{#1} \hfil
\epsfxsize=.45\textwidth \epsfbox{#2}}
\def\plotfiddle#1#2#3#4#5#6#7{\centering \leavevmode
\vbox to#2{\rule{0pt}{#2}}
\special{psfile=#1 voffset=#7 hoffset=#6 vscale=#5 hscale=#4 angle=#3}}
\def\ltsima{$\;\buildrel<\over\sim\;$}
\def\simlt{\lower.5ex\hbox{\ltsima}}
\def\gtsima{$\;\buildrel>\over\sim\;$}
\def\simgt{\lower.5ex\hbox{\gtsima}}

%%%%% For units of measure %%%%%
%
\def\dynpercm{\nobreak\mbox{$\;$dynes\,cm$^{-1}$}}
\def\cmpermin{\nobreak\mbox{$\;$cm\,min$^{-1}$}}
%
%%%%%

%%%%% For dimensionless numbers %%%%%
%
\def\Real{\mbox{Re}}      % cf plain TeX's \Re and Reynolds number
\def\Imag{\mbox{Im}}      % cf plain TeX's \Im
\def\Rey{\mbox{\it Re}}   % Reynolds number
\def\Pran{\mbox{\it Pr}}  % Prandtl number, cf plain TeX's \Pr product
\def\Pen{\mbox{\it Pe}}   % Peclet number
\def\Ai{\mbox{\it Ai}}    % Airy function
\def\Bi{\mbox{\it Bi}}    % Airy function
%
%%%%%


%%%%% For authors without AMSTeX %%%%%
%
% Uncomment the definitions as far as: %%% STOP HERE without AMSTeX %%%
%
\def\upi{\pi} % to be replaced with upright Greek character
\def\umu{\mu} % to be replaced with upright Greek character
\def\BbbE{\mbox{\sf E}} % to be replaced with blackboard bold
\def\blackbox{\rule{4pt}{4pt}} % to be replaced with \blacksquare
%
%%%%% STOP HERE without AMSTeX %%%%%

\def\hexnumber#1{\ifcase#1 0\or1\or2\or3\or4\or5\or6\or7\or8\or9\or
 A\or B\or C\or D\or E\or F\fi }

%%%%% For authors with AMSTeX %%%%%
%
% Uncomment the definitions as far as %%% STOP HERE with AMSTeX %%%
%
% Example font defns for AMS Euler fonts for upright Greek characters
%
% \font\eurmten=eurm10
% \font\eurmseven=eurm10 at 7pt
% \font\eurmfive=eurm10 at 5pt
% \newfam\eurmfam
% \textfont\eurmfam=\eurmten
% \scriptfont\eurmfam=\eurmseven
% \scriptscriptfont\eurmfam=\eurmfive
% \edef\eurm@{\hexnumber\eurmfam}
%
% \mathchardef\upi="0\eurm@19   % for upright Greek character
% \mathchardef\umu="0\eurm@16   % for upright Greek character
%
% \font\msxten=msam10
% \font\msxseven=msam10 at 7pt
% \font\msxfive=msam10 at 5pt
% \newfam\msxfam
% \textfont\msxfam=\msxten
% \scriptfont\msxfam=\msxseven
% \scriptscriptfont\msxfam=\msxfive
% \edef\msx@{\hexnumber\msxfam}
%
% \mathchardef\leqslant="3\msx@36
% \mathchardef\geqslant="3\msx@3E
% \let\le=\leqslant
% \let\ge=\geqslant
% \let\leq=\leqslant
% \let\geq=\geqslant
%
% \def\BbbE{\Bbb E}
% \def\blackbox{\blacksquare}
% \renewcommand{\simeq}{\approx}
%
%%%%% STOP HERE with AMSTeX %%%%%


%%%%% For sans serif characters %%%%%
%
\def\ssC{\mbox{\sf C}}         % for sans serif C
\def\sfsP{\mbox{\sfs P}}       % for sans serif sloping P
\def\slsQ{\mbox{\sls Q}}       % for sans serif bold-sloping Q
%
\makeatletter
\ifx\CUP@mtlplain@loaded\undefined
  \font\sfs = cmssi10    % sans-serif slanted
  \font\sfb = cmssi10    % sans-serif bold maths
  \font\sls = cmssi10    % sans-serif bold maths, slanted
  \font\bit = cmmib10    % bold math italic
\else
  % CUP times font substitutions for above (not to be used by authors)
  \font\sfs = mtssi10    % sans-serif italic
  \font\sfb = mtssbx10   % sans-serif bold maths
  \font\sls = mtssbi10   % sans-serif bold maths, slanted
  \font\bit = mtmib10    % bold math italic
\fi
\makeatother
%
%%%%%


%%%%% Hat position %%%%%
%
% \def\hatp{\skew5\hat{p}}        % p with hat
% \def\hatR{\skew5\hat{R}}        % R with hat
% \def\hatRR{\skew5\hat{\hatR}}   % R with 2 hats
% \def\doubletildesigma{\skew5\tilde{\skew5\tilde{\sSigma}}}
%               italic Sigma with double tilde
%%%%%


%%%%% FOR MATH BOLD ITALIC %%%%%
%
% if you need math bold italic uncomment to END MATH BOLD ITALIC
%
 \makeatletter
 \ifx\CUP@mtlplain@loaded\undefined
   \font\tenbmi=cmmib10 at 10pt
   \font\sevenbmi=cmmib10 at 7pt
   \font\fivebmi=cmmib10 at 5pt

   \newfam\bmifam
   \textfont\bmifam=\tenbmi
   \scriptfont\bmifam=\sevenbmi
   \scriptscriptfont\bmifam=\fivebmi
   \def\bmi{\fam\bmifam\tenbmi}
 \fi
 \makeatother
%
%%%%% END MATH BOLD ITALIC %%%%%

\ifnfsstwo
  \newcommand{\mitbf}[1] {\hbox{\mathversion{bold}$\mathit{#1}$}}
  \newcommand{\rmn}[1] {{\mathrm #1}}
  \newcommand{\itl}[1] {{\mathit #1}}
\fi
\ifnfssone
  \newcommand{\mitbf}[1] {{\mathversion{bold}\mathit{#1}}}
  \newcommand{\rmn}[1] {{\normalshape #1}}
  \newcommand{\itl}[1] {{\mathit #1}}
\fi
\ifoldfss
  \newcommand{\mitbf}[1] {\mbox{\boldmath $#1$}}
  \newcommand{\rmn}[1] {{\rm #1}}
  \newcommand{\itl}[1] {{\it #1}}
\fi

\newcommand{\GaPQ}  {G_a(P,Q)}
\newcommand{\Gat}   {\widetilde{G_a}}
\newcommand{\GsPQ}  {G_s(P,Q)}
\newcommand{\kgd}   {k\gamma d}
\newcommand{\ndq}   {\frac{\mbox{$\partial$}}{\mbox{$\partial$} n_q}}
\newcommand{\p}     {\mbox{$\partial$}}
\newcommand{\sh}    {^{\shalf}}
\newcommand{\smh}   {^{-\shalf}}
\newcommand{\sumjm} {\sum_{j=1}^{M}}
\newcommand{\tti}   {\rightarrow\infty}
\newcommand{\ttz}   {\rightarrow 0}
\mathchardef\varLambda="0103


%%%%% The minus sign is in different positions for the two fonts %%%%%
%
\makeatletter
\ifx\CUP@mtlplain@loaded\undefined
  \newcommand{\pvi}{\int_0^{\infty}\mskip -33mu -\quad} % 33mu for cm
\else
  \newcommand{\pvi}{\int_0^{\infty}\mskip -30mu -\quad} % 30mu for mt
\fi
\makeatother
%
%%%%%


%%%%% Bold Math Symbols %%%%%
%
\makeatletter
\ifx\CUP@mtlplain@loaded\undefined
  \font\tenbms=cmbsy10
  \font\sevenbms=cmbsy10 at 7pt
  \font\fivebms=cmbsy10 at 5pt
%
  \newfam\bmsfam
  \textfont\bmsfam=\tenbms
  \scriptfont\bmsfam=\sevenbms
  \scriptscriptfont\bmsfam=\fivebms
%
  \def\bms{\fam\bmsfam\tenbms}
  \edef\bsy@{\hexnumber\bmsfam}
  \mathchardef\bnabla="0\bsy@72
\fi
\makeatother
%
%%%%%

\def\eg{{e.g.\ }}
\def\etc{{etc.\ }}
\def\etal{\mbox{\it et al.}}

\newcommand{\thalf}{\textstyle\frac{1}{2}}
\newcommand{\shalf}{\scriptstyle\frac{1}{2}}
\newcommand{\squart}{\frac{1}{4}}
\newcommand{\etb}{\hbox{\boldmath$\eta$}}
%\newcommand{\etbox}{$\eta$} % use this if your \boldmath doesn't work.
\newcommand{\biS}{\bit S}

% array strut to make delimiters come out right size both ends
\newcommand{\astrut}{\rule[-5pt]{0pt}{20pt}}

\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}

% use these four lines when finally presenting your CRC. (See Appendix B
% of the guide.)
% \magnification    1200  % always use 1200 when presenting your chapter
%\magnification    1150  % always use 1200 when presenting your chapter
%\oddsidemargin  -0.5pc  % appropriate for A4, you may need to vary value
%\evensidemargin -0.5pc  % appropriate for A4, you may need to vary value
%\topmargin        -5pc  % appropriate for A4, you may need to vary value
%\topmargin        -2pc  % appropriate for 8x11 inch paper
%\topmargin        -2.5pc  % appropriate for 8x11 inch paper
%\topmargin          -1pc  % appropriate for 8x11 inch paper

